Semantic Similarity Models for Depression Severity Estimation

Depressive disorders constitute a severe public health issue worldwide. However, public health systems have limited capacity for case detection and diagnosis. In this regard, the widespread use of social media has opened up a way to access public information on a large scale. Computational methods can serve as support tools for rapid screening by exploiting this user-generated social media content. This paper presents an efficient semantic pipeline to study depression severity in individuals based on their social media writings. We select test user sentences for producing semantic rankings over an index of representative training sentences corresponding to depressive symptoms and severity levels. Then, we use the sentences from those results as evidence for predicting users' symptom severity. For that, we explore different aggregation methods to answer one of four Beck Depression Inventory (BDI) options per symptom. We evaluate our methods on two Reddit-based benchmarks, achieving 30\% improvement over state of the art in terms of measuring depression severity.

==> sections/JAVI-Revised-Reviewer1.tex <==
First, we thank the reviewer for their feedback regarding our submission. We have done our best to address all the comments. We will comment point by point on our revisions. We are convinced that the revised manuscript will improve over the previous version, particularly in the experimental analysis and further general explanations. The reviewer's appreciation has greatly contributed to this improvement.

We appreciate its feedback on the paper, highlighting that our approach was interesting to the reviewer and that the manuscript is generally well-written.

We will comment point by point on our revisions:

**Comment 1: the actual use case or scenario in which the approach should be applied is not clear/motivated.

--Response 1:
We will clarify this idea at the beginning of Subsection 5.2 (Interpretability - Case Study). We first mention recent works highlighting the importance of using clinical markers that can facilitate their interpretation by health professionals. By doing so, mental health detection models may be better integrated into clinical settings. This motivation aligns with our Introduction in Section 1, where we discussed the need for interpretability in the predictions of mental health detection models.
In our case study, we show how inspecting for the presence of specific symptoms can be clear candidates for interpretable clinical markers. For this purpose, in Tables 7 and 8, we present paraphrased publications of test users that our method highlighted. These examples include the symptoms of "Sleep problems" and "Loss of Pleasure". A good scenario where our approach can be applied is as a pre-screening method for users with potentially concerning publications based on symptom risks. As we comment in Subsection 5.2, these health professionals may inspect sentences as a first step towards further diagnosis or monitoring methods during treatment.

**Comment 2: it is not clear whether the (slight) improvements over the other methods actually are practically useful in the sense that it is not discussed what effectiveness level would be needed for some clinician to actually use some automatic support like the one presented; for instance, the reported RMSE scores in Table 4 seem to indicate that the lower three BDI depression levels are less wide than the actual RMSE ... how is such a system useful at all? -> why shouldn't clinicians not just simply let a person complete the actual questionnaire?!

--Response:
We may not have understood the RMSE comment from the reviewer. In Table 4, we are not reporting severity levels, and RMSE values are computed over the final score of the BDI score, that is, in a range of 0 to 63. We know that there is room for improvement in terms of RMSE. However, the effect of each error on RMSE is proportional to the size of the squared error; thus, larger errors have a disproportionately large impact on the metric. In any case, the RMSE values do not indicate by themselves where the error relies on terms of the depression severity of the individuals. Table 6 (a) shows that information, showing the F1 values for the different severity levels. These numbers present differences among the categories, but in a positive way. That is, we get the best values on the more severely depressed individuals, who may be at a higher risk, and it may be a problem not to contact them. This domain is a clear case where false positives are less problematic than false negatives (e.g. contacting an individual that is fine for checking out should not be so problematic as ignoring an individual with severe depression).
Regarding the question of why clinics should not just let people fill out these questionnaires:
Many health organisations also make these questionnaires available to users for self-completion. These online tests may even advise you to see a doctor. Conventional procedures, on the other hand, may have significant limitations when attempting to make a precise global diagnosis. Disclosing your mental illnesses remains a complicated and stigmatised process. Furthermore, respondents can easily manipulate the total score of the questionnaires. Existing research has examined how these responses can vary dramatically depending on the changing factor [1,2]. On the other hand, it has been found that young people are more prone to discuss sensitive issues online than face-to-face [3]. For this reason, using this type of user-generated data to fill these questionnaires may be a promising approach.

**Comment 3: other methods reported in the paper sometimes perform equally well or only very slightly worse (e.g., why isn't the RMSE of CYUT in bold for eRisk 2021 in Table 4); since effect size and practically needed effect size is not discussed, it is difficult to actually assess the contribution.

--Response 3:
We thank the reviewer for the suggestions. As the primary metric relies on an ordered categorical variable (DCHR is the percentage of subjects that were correctly categorised in one of the four levels: minimal, mild, moderate and severe) to perform classical statistical tests, we used the per-user category severity error (i.e. by how many levels the model missed). Using the permutation tests (1M of permutations) for that DCHR error, we found, for instance, in the case of the eRisk 2020, the following p-values: ILab: 0.038572961427038574, BioInfo: 0.000374999625000375, RELAI: 0.09675690324309676 and UPV: 0.010455989544010455. We will include the results in the revised version of the paper.

**Comment 4: how well do large language models work on the task when prompted "appropriately"? (e.g., GPT-3 or ChatGPT)

--Response 4:
This is an exciting experiment that we keep in mind! However, we have yet to explore it. Answering your question, we are aware that Nguyen et al. [4] recently presented their findings on this topic at ACL 2022, where they compared (1) BERT-based classifiers and (2) GPT-3 with prompted examples in the context of mental health detection. However, the high computational cost of GPT-3 makes it challenging to provide sufficient prompts for such a complex task. For this reason, Nguyen et al. prompted GPT-3 with only four examples for positive and negative classes and evaluated it on 100 positive and 100 negative samples. GPT-3 performed worse in comparison with BERT-classifiers. However, these models are highly dependent on the quality of the prompts, so this comparison is difficult to assess. Given these reasons and that we do not have as much computing power, a thorough evaluation of this idea is beyond the scope of our paper, and we plan to consider it in future research.

**Comment 5: place tables at the top of columns?!,  rather spell out WH!?

--Response:
Solved! Thanks. We will use the term writing history in the updated manuscript instead of WH.

[1] Cameron, Isobel M., et al. "Measuring depression severity in general practice: discriminatory performance of the PHQ-9, HADS-D, and BDI-II." British Journal of General Practice 61.588 (2011): e419-e426.
[2] Bowling, Ann. "Mode of questionnaire administration can have serious effects on data quality." Journal of public health 27.3 (2005): 281-291.
[3] Kauer, S. D., Mangan, C., & Sanci, L. (2014). Do online mental health services improve help-seeking for young people? A systematic review. Journal of medical Internet research, 16(3), e3103.
[4] Thong Nguyen, Andrew Yates, Ayah Zirikly, Bart Desmet, and Arman Cohan. 2022. Improving the generalizability of depression detection by leveraging clinical questionnaires. In Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers), ACL 2022, Dublin, Ireland, May 22-27, 2022, pages 8446-8459. Association for Computational Linguistics.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECOND REBUTTAL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Responses 1 and 2: I am still not sure what the actual use case of the suggested approach is and hence am also not sure about how "important" the slight improvements of the new approach actually are. I would suggest to really describe the use case in the introduction to motivate the scenario in which the approach would be applied. For instance, is the goal (1) a tool that constantly monitors social media posts from people and then suggests to see a clinician when the detected depression level is too high? Or is the goal (2) an add-on tool for a clinician to prepare for an appointment with a person that already contacted them and that agreed to share their social media or whatever history? In case of (1), I would then be interested in what effectiveness of the detection tool would be needed so that people would accept the respective "visit a doctor" suggestions. In case of (2), I somewhat question whether the actual depression level would really be needed to be estimated since the actual clinician then probably would only be interested in finding the actual textual evidences that signal depression problems (since they probably already asked the person to fill the questionnaire that then probably also signaled some higher depression risk).


%% Response 1 is more about the use case of the whole technique (but simply your approach): Why do we need such depression detection? The reviewer mentioned two potential use cases and also addressed further concerns. I think it is better to edit your rebuttal to answer his concern.


% Tengo 3 papers recientes (ACL, IJCAI y WWW) con metodos parecidos, 2 basados en sintomas y otro para estimar niveles de depresion. Tengo una review reciente de un paper de como aprovechar "Using Social Media for Mental Health Surveillance: A Review". 

%Although the proposed method provides strong performance for questions of internal validity, however, external validity, i.e., testing in a clinical settings [18] is unproven because we only analyze posts on Reddit and do not interact with the user experience. Further, our work focuses on developing a computational method for screening users and is not intended to use in clinical settings to make any diagnostic claims related to depression


Response 1 and 2:

The implications of this research posit numerous social benefits – in new monitoring and public health efforts, designing interventions for dangerous behaviours, and the potential to improve health and well-being [9, 10]. Some clear examples are those the reviewer proposed (goals 1 and 2). However, as the reviewer commented, we understand that applying this type of proposal in real scenarios requires much study and analysis due to future flaws. These types of NLP models should not be immediately transferred to decision support systems. Further studies with participant recruitment, trials and regulatory approval would be needed.

Despite the gap between mental health prediction models and actual clinical practice, many recent studies like ours investigated approaches to identifying and detecting depression using reliable clinical markers. These studies seek to propose solutions that can be a proxy between health professionals and NLP methods. Some examples are the works of Nguyen et al. ACL 2022 [5], Zhang et al. IJCAI 2022 [6] or Naseem et al. WWW 2022 [7] that, also evaluated the effectiveness of their proposals in eRisk collections. Our study aims to contribute to this area of research and advance the development of reliable solutions for health professionals.

As we argued in the previous comment, assessing depression is difficult in practical settings: even experienced clinicians struggle to interpret signals [8], and the administration of questionnaires is far from perfect. However, our work is a step towards developing models that help scalable tools to mitigate individual risk. The motivation of previous articles provides a good context for what these models can contribute, and it has served as an inspiration to develop approaches that rely on clinically validated schemas (such as our model with the BDI-II questionnaire).

Answering the concerns about the reviewer's ideas (1) and (2):
Goal (1) may be perfectly reasonable (within the obvious limitations of these imperfect models). However, answering the comment, "I would then be interested in what effectiveness of the detection tool would be needed so that people would accept the respective "visit a doctor" suggestions", is beyond our reach. There is a lot of uncertainty as to what extent these models can be effective in that case. In the case of goal (2), "I somewhat question whether the actual depression level would really be needed to be estimated since the actual clinician then probably would only be interested in finding the actual textual evidence that signal depression problems", this scenario would be different. If we consider that a clinician has already diagnosed an individual with depression, we believe that the use of our approach as monitoring would be better suited. In this case, the clinician could revise the evolution of specific symptoms' severity to help them better understand their patient's context.

Response 3:
We understand that this response aligns with the comments in Responses 1 and 2, and our previous statement can help better understand the reviewer's concerns. It is very complex to demonstrate from what effectiveness score our model may be clinically helpful. We should have clarified that the efficacy of the severity markers from depression varies greatly even when used by human therapists [11]. There is a lot of disagreement when using different questionnaires. Korner et al. [11] investigated the inter-correlation of depression scales using different questionnaires. In some cases, health professionals have even less agreement when using different instruments than the agreement between the predictions of our model and the golden truth (e.g. spearman inter-correlation of scales of 0.21 between DSM and Hamilton Depression Scale [11]). 

Answering reviewer concerns: In the use case scenario (1), evaluating that our method can detect evidence before others would be an interesting experiment. We know that there are other eRisk collections dedicated exclusively to early risk detection. However, these collections correspond to a binary setting (depressive vs non-depressive users). For this reason, adapting our model to this setting is beyond the scope of the article. We will consider it in future work. In the case of scenario 2, demonstrating that our model can detect better evidence than previous approaches is also complicated. As we showed in section 5.2 (Interpretability - Case Study), our method offers evidence and interpretability based on the presence of BDI symptoms. Previous eRisk works did not pursue the highlighting of user publications that lead to every symptom decision, so this comparison can not be made (and again, it would be needed to consider a fair comparison between different approaches).


[1] Cameron, Isobel M., et al. "Measuring depression severity in general practice: discriminatory performance of the PHQ-9, HADS-D, and BDI-II." British Journal of General Practice 61.588 (2011): e419-e426.

[2] Bowling, Ann. "Mode of questionnaire administration can have serious effects on data quality." Journal of public health 27.3 (2005): 281-291.

[3] Kauer, S. D., Mangan, C., & Sanci, L. (2014). Do online mental health services improve help-seeking for young people? A systematic review. Journal of medical Internet research, 16(3), e3103.

[4] Thong Nguyen, Andrew Yates, Ayah Zirikly, Bart Desmet, and Arman Cohan. 2022. Improving the generalizability of depression detection by leveraging clinical questionnaires. In Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers), ACL 2022, Dublin, Ireland, May 22-27, 2022, pages 8446-8459. Association for Computational Linguistics.

[5] Thong Nguyen, Andrew Yates, Ayah Zirikly, Bart Desmet, and Arman Cohan. 2022. Improving the generalizability of depression detection by leveraging clinical questionnaires. In Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers), ACL 2022, Dublin, Ireland, May 22-27, 2022, pages 8446-8459. Association for Computational Linguistics.

[6] Zhiling Zhang, Siyuan Chen, Mengyue Wu, and 877 Kenny Q. Zhu. 2022a. Psychiatric scale guided risky post screening for early detection of depression. In Proceedings of the Thirty-First International Joint Conference on Artificial Intelligence, IJCAI 2022, Vienna, Austria, 23-29 July 2022, pages 5220–5226. 
ijcai.org

[7] Naseem, Usman & Dunn, Adam & Kim, Jinman & Khushi, Matloob. (2022). Early Identification of Depression Severity Levels on Reddit Using Ordinal Classification. 2563-2572. 10.1145/3485447.3512128. 

[8] COPPERSMITH, Glen, et al. Natural language processing of social media as screening for suicide risk. Biomedical informatics insights, 2018, vol. 10, p. 1178222618792860.

[9] Stevie Chancellor, Eric P. S. Baumer, and Munmun De Choudhury. 2019. Who is the "Human" in Human-Centered Machine Learning: The Case of Predicting Mental Health from Social Media. Proc. ACM Hum.-Comput. Interact. 3, CSCW, Article 147 (November 2019), 32 pages. https://doi.org/10.1145/3359249

[10] Skaik, Ruba, and Diana Inkpen. "Using social media for mental health surveillance: a review." ACM Computing Surveys (CSUR) 53.6 (2020): 1-31.

[11] Kørner, A., et al. "Quantifying depressive symptomatology: inter-rater reliability and inter-item correlations." Journal of affective disorders 20.2 (1990): 143-149.

==> sections/JAVI-Revised-Reviewer2.tex <==
First, we thank the reviewer for their feedback regarding our submission. We have done our best to address all the comments. We will comment point by point on our revisions. We are convinced that the revised manuscript is improved over the previous versions, particularly in the experimental analysis and further general explanations. The reviewer's appreciation has greatly contributed to this improvement.

We value its feedback on the paper. We are pleased that you found the retrieval-based baselines and their interpretation novel. Moreover, we are also happy that the reviewer considered our experiments and analyses solid.

We will comment point by point on our revisions:

**Comment 1: The paper did not report the robustness and significance level.

--Response 1:
We thank the reviewer for the suggestions. As the primary metric relies on an ordered categorical variable (DCHR is the percentage of subjects that were correctly categorized in one of the four levels: minimal, mild, moderate and severe) to perform classical statistical tests, we used the per-user category severity error (i.e. by how many levels the model missed). Using the permutation tests (1M of permutations) for that DCHR error, we found, for instance, in the case of the eRisk 2020, the following p-values: ILab: 0.038572961427038574, BioInfo: 0.000374999625000375, RELAI: 0.09675690324309676 and UPV: 0.010455989544010455. We will include the results in the revised version of the paper.

**Comment 2: The writing can be further improved

--Response 2:
We have inspected the article again to improve the clarity and coherence of our writing. Overall, we have focused on enhancing Section 3 (Method), including the explanation of our two main components: Section 3.1 (Semantic Retrieval Pipeline) and Section 3.2 (Silver Sentences Selection).

**Comment 3:
Missing References:
The following (earlier) works quantify, predict, and further analyzes the severity (changes) of mental illness over time with NLP techniques.
Li et al., 2018, Text-Based Detection and Understanding of Changes in Mental Health, SocInfo 2018.
Gaur et al., 2021, Characterization of time-variant and time-invariant assessment of suicidality on Reddit using C-SSRS, PLOS ONE 2021.

--Response 3:
Thanks for the suggestion! We will look into these works and refer to similar studies considering different severity levels for mental health detection models.

==> sections/JAVI-Revised-Reviewer3.tex <==
First, we thank the reviewer for their feedback regarding our submission. We have done our best to address all the comments. We will comment point by point on our revisions. We are convinced that the revised manuscript is improved over the previous versions, particularly in the experimental analysis and further general explanations. The reviewer's appreciation has greatly contributed to this improvement.

We appreciate its feedback on the paper, considering that our approach can be interpretable and explainable, and this fact can be helpful in clinical settings with appropriate validation of clinicians.

We will comment point by point on our revisions:

**Comment 1: Sentence-level evaluation of the proposed method seems weak. Although Sec 5.1 and 5.2 discusses the quality of retrieved posts with only a handful of samples, a quantitative evaluation would be needed to assess how well different approaches in "silver sentence generation" retrieved similar posts. Manual annotations (such as the one carried out in the Aug Dataset approach) of sample silver sentences could be an option.

--Response 1:
Thanks for the suggestion. To get statistics on a quantitative evaluation of our sentence selection models, we will use the manual annotations, as you point out. In specific, a total of 17.15% were annotated as positives from the pool of candidate sentences. We will incorporate these results in the revised version of the paper.

**Comment 2: It is less discussed why the proposed method did not perform great with the larger dataset (eRisk 2021). Table 4 shows that the proposed methods outperformed the prior methods in the DCHR metric only. Furthermore, the proposed methods performed almost similarly between eRisk 2020 and 2021, even though the eRisk 2021's training set is nearly five times larger than that of 2020. Intuitively speaking, a retrieval-based method could work better if the source dataset was larger because there would be more relevant examples. Does this mean the proposed method would not improve performance by increasing the size of training data?

--Response 2:
We agree that intuitively, a retrieval system should improve its performance as training data increases. However, in a domain as complex as the detection of depression severity levels, it can be very difficult to obtain more general results. This has also been the case for the other participants in the eRisk collection, as most of the models have worsened results for the eRisk 2021 collection (for more details, please refer to the eRisk 2020 and 2021 working notes [1,2]).
In turn, a recent study has demonstrated this problem of generalisation to different collections for these types of mental health detection models [3]. For this reason, we believe that not worsening the results, if not maintaining them, is not as strange a phenomenon as it might be in collections of a more standard nature.

**Comment 3: a) The terminology needs to be more accurate.
The symptom's severity scale is referred to as different words, 'option' and 'label', without notice. One coherent term is preferred for readability. "Silver sentence generation" (Sec 3.2 ) does not generate texts from scratch (like by using text generation models) but labels a pool of existing sentences afterwards. Consider using "distant supervision" or similar terms instead of "generation'.

--Response3 : 
We have changed our terminology to make the article easier to read. Regarding the term referred to the severity scale of a symptom, we now use the word "label" consistently. Moreover, we clarify this terminology in Footnote 3 (Page 3 of the manuscript). Regarding the silver generation title, thank you for this appreciation! We agree that this term can generate confusion with text generation models. Therefore, we have changed the name of our sentence selection method. We have also changed the title of our sentence selection method (Subsection 3.2, now renamed to Silver Sentences Selection). 

**Comment 4: b) What semantic similarity method was adopted in the "Aug Dataset" approach for "silver sentence generation"? Is it the same RoBERTa used in the "semantic retrieval pipeline"?

--Response 4:
Yes, we have used the same similarity method to augment silver sentences, a missing detail in the original manuscript. The revised version now includes an explicit mention of this important information.

**Comment 5: c) The gold sentences (35 labelled sentences per symptom) could be made public to contribute to the community.

--Response:
 Yes, we agree that this dataset may help develop depression detection models. We are currently working on a manuscript where we extend and analyse this resource in more detail. Following eRisk policies (the eRisk collections are the original data source), and due to the sensitivity of the data, the extended dataset will only be available under a research data agreement.

**Comment 6: d) In Table 4, the best RMSE in eRisk 2021 is 12.78 of CYUT, although 14.17 by a proposed method (Accum Voting SBERT) is marked in bold.

-Response 6:
We apologise for the error. The revised paper now correctly displays the best RMSE, highlighted in bold, for CYUT.

**Comment 7: e) The discussion in Sec 5 should include ADODL and ACR. (On the other hand, the oracle experiment for AHR was very informative.)
Response:

--The ADODL is the Difference Between Overall Depression Levels (DODL) averaged over all users. DODL does not look at question-level hits or differences but computes the overall depression level (sum of all the answers) for the real and automated questionnaires. Next, the absolute difference (ad overall) between the real and the predicted score is computed. Depression levels are integers between 0 and 63; thus, DODL is normalised into [0,1] as follows: DODL = (63 − ad overall)/63. For this metric, in eRisk2020, our proposed methods outperform all prior work. Similar to other metrics, our results are more modest in the eRisk2021 collection. This metric is similar to the RMSE, which considers the total error between the real and predicted questionnaires. We considered not discussing this metric for page limit constraints in the Section. The ACR is the Closeness Rate (CR) averaged over all users. CR takes into account that the answers to the depression questionnaire represent an ordinal scale. Imagine that the actual user answered" 0". A system S1, whose answer is" 3", should be penalised more than a system S2, whose answer is" 1". For each question, CR computes the absolute difference (ad) between the real and the predicted answer (e.g. ad=3 and ad=1 for S1 and S2, respectively) and, next, this absolute difference is transformed into an effectiveness score as follows: CR = (mad − ad)/mad, where mad is the maximum absolute difference, which is equal to the number of possible answers minus one. As we argued in Section 5 (Results), we decided to focus more on assessing overall depression levels (DCHR metric) than focusing on specific symptoms. 

**Comment 8:  f) The term "significantly" (at Line 554) should not be used in results/discussion sections unless it means statistically significant with a statistical test.

--Response:
 We agree that this term needs to be clarified. We will remove it in the updated version of the article. Thanks again for going into so much detail.

**Comment 9:  g) Table 7's "Golden option" and "Predicted option" columns look the other way around according to the corresponding body text (Sec 5.2; the description at Line 560-561 does not match the table's values).

Response:
That is correct. We apologise for the mistake. In the updated version, you will find the corrected column names.

[1] Losada, David E., Fabio Crestani, and Javier Parapar. "Overview of eRisk at CLEF 2020: Early Risk Prediction on the Internet (Extended Overview)." CLEF (Working Notes) (2020).
[2] Parapar, J., Martín-Rodilla, P., Losada, D. E., & Crestani, F. (2021). Overview of eRisk at CLEF 2021: Early Risk Prediction on the Internet (Extended Overview). CLEF (Working Notes), 864-887.
[3] Harrigian, Keith, Carlos Aguirre, and Mark Dredze. "Do models of mental health based on social media data generalise?." Findings of the association for computational linguistics: EMNLP 2020. 2020.

==> sections/XX-Reviewers-Responses.tex <==
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! REVIEWER 1 !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 

First, we thank the reviewer for her/his feedback regarding our submission. We have done our best to address all the comments. We will comment point by point on our revisions. We are convinced that the revised manuscript is gonna be an improvement over the previous versions, particularly in the experimental analysis and further general explanations. The reviewer's appreciation has greatly contributed to this improvement. 

We appreciate its feedback on the paper, highlighting that our approach was interesting to the reviewer and that the manuscript is generally well-written.

We will comment point by point on our revisions:

Comment 1: the actual use case or scenario in which the approach should be applied is not clear/motivated.

Response:

We will clarify this idea at the beginning of Subsection 5.2 (Interpretability - Case Study). We first mention recent works highlighting the importance of using clinical markers easily interpretable by health professionals. By doing so, mental health detection models may be better integrated into clinical settings. This aligns with our Introduction in Section 1, where we discussed the need for interpretability in the predictions of mental health detection models.

In our case study, we show how inspecting for the presence of certain symptoms can be clear evidence of clinical markers. 
For this purpose, in Tables 7 and 8, we present paraphrased publications of test users that were highlighted by our method. These examples include the symptoms of "Sleep problems" and "Loss of Pleasure". Our approach allows for screening users with potentially concerning publications based on symptom risks, which can then be reviewed by healthcare professionals. As we comment in Subsection 5.2, these health professionals may inspect sentences as a first step towards further diagnosis or monitoring methods during treatment.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comment 2: it is not clear whether the (slight) improvements over the other methods actually are practically useful in the sense that it is not discussed what effectiveness level would be needed for some clinician to actually use some automatic support like the one presented; for instance, the reported RMSE scores in Table 4 seem to indicate that the lower three BDI depression levels are less wide than the actual RMSE ... how is such a system useful at all? -> why shouldn't clinicians not just simply let a person complete the actual questionnaire?!

Response:

We are not sure about the RMSE comment from the reviewer. In Table 4 we are not reporting severity levels, and RMSE values are computed over the final score of the BDI, that is, in a range of 0 to 63. We know that there is room for improvement in terms of RMSE. However, the effect of each error on RMSE is proportional to the size of the squared error; thus larger errors have a disproportionately large effect on the metric. In any case, the RMSE values do not indicate by themselves where the error relies on terms of the depression severity of the individuals.  That information can be found in Table 6 (a) where we show the F1 values for the different severity levels. These numbers show differences among the results, but in a positive way, that is, we get the best values on the more severely depressed individuals, those that may be at a higher risk and it may be a problem to not contact them. This domain is a clear case where false positives are less problematic than false negatives (e.g. contacting an individual that is fine for checking out should not be so problematic as ignoring an individual with severe depression). 

Regarding the question of why clinics should not just let people fill out these questionnaires: 

Many health organizations also make these questionnaires available to users for self-completion. These online tests may even advise you to see a doctor. Conventional procedures, on the other hand, may have significant limitations when attempting to make a precise global diagnosis. Disclosing your mental illnesses remains a difficult and stigmatized process. Furthermore, respondents can easily manipulate the total score of the questionnaires. Existing research has examined how these responses can vary dramatically depending on the changing factor [1,2]. On the other hand, it has been found that young people are more prone to discuss sensitive issues online
than face-to-face [3]. For this reason, using this type of user-generated data to fill these questionnaires may be a promising approach.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comment 3: other methods reported in the paper sometimes perform equally well or only very slightly worse (e.g., why isn't the RMSE of CYUT in bold for eRisk 2021 in Table 4); since effect size and practically needed effect size is not discussed, it is difficult to actually assess the contribution.

Response:

We thank the reviewer for the suggestions. As the main metric relies on an ordered categorical variable (DCHR is the percentage of subjects that were correctly categorized in one of the four levels: minimal, mild, moderate and severe) to perform classical statistical tests, we used the per-user category severity error (i.e. by how many levels the model missed). Using the permutation tests (1M of permutations) for that DCHR error, we found, for instance, in the case of the eRisk 2020, the following p-values: ILab: 0.038572961427038574, BioInfo: 0.000374999625000375, RELAI: 0.09675690324309676 and UPV: 0.010455989544010455. We will include the results in the revised version of the paper. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comment 4: how well do large language models work on the task when prompted "appropriately"? (e.g., GPT-3 or ChatGPT)

Response:

This is an exciting experiment that we keep in mind! However, we have not explored it yet. Answering your question, we are aware that Nguyen et al. [4] recently presented their findings on this topic at ACL 2022, where they compared (1) BERT-based classifiers and (2) GPT-3 with prompted examples in the context of mental health detection. However, the high computational cost of GPT-3 makes it challenging to provide a sufficient number of prompts for such a complex task. For this reason, Nguyen et al. prompted GPT-3 with only four examples for positive and negative classes and evaluated it on 100 positive and 100 negative samples. GPT-3 performed worse in comparison with BERT-classifiers. However, these models are highly dependent on the quality of the prompts, so this comparison is difficult to assess. Given these reasons and that we do not have as much computing power, we believe a thorough evaluation of this idea is beyond the scope of our paper, and we plan to consider it in future research.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comments, Suggestions and Typos:

Comment 5: place tables at the top of columns?!

Response:

Solved! Thanks


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comment 6: rather spell out WH!?

Response:

In the updated manuscript, we will use the term writing history instead of WH.


[1] Cameron, Isobel M., et al. "Measuring depression severity in general practice: discriminatory performance of the PHQ-9, HADS-D, and BDI-II." British Journal of General Practice 61.588 (2011): e419-e426.

[2] Bowling, Ann. "Mode of questionnaire administration can have serious effects on data quality." Journal of public health 27.3 (2005): 281-291.

[3] Kauer, S. D., Mangan, C., & Sanci, L. (2014). Do online mental health services improve help-seeking for young people? A systematic review. Journal of medical Internet research, 16(3), e3103.

[4] Thong Nguyen, Andrew Yates, Ayah Zirikly, Bart Desmet, and Arman Cohan. 2022. Improving the generalizability of depression detection by leveraging clinical questionnaires. In Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers), ACL 2022, Dublin, Ireland, May 22-27, 2022, pages 8446-8459. Association for Computational Linguistics.



% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! REVIEWER 2 !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 


First, we thank the reviewer for her/his feedback regarding our submission. We have done our best to address all the comments. We will comment point by point on our revisions. We are convinced that the revised manuscript is improved over the previous versions, particularly in the experimental analysis and further general explanations. The reviewer's appreciation has greatly contributed to this improvement. 


We value its feedback on the paper. We are pleased that you found the retrieval-based baselines and their interpretation to be novel. Moreover, we are also pleased that the reviewer considered our experiments and analyses solid.


We will comment point by point on our revisions:


Comment 1: The paper did not report the robustness and significance level.

Response:

We thank the reviewer for the suggestions. As the main metric relies on an ordered categorical variable (DCHR is the percentage of subjects that were correctly categorized in one of the four levels: minimal, mild, moderate and severe) to perform classical statistical tests, we used the per-user category severity error (i.e. by how many levels the model missed). Using the permutation tests (1M of permutations) for that DCHR error, we found, for instance, in the case of the eRisk 2020, the following p-values: ILab: 0.038572961427038574, BioInfo: 0.000374999625000375, RELAI: 0.09675690324309676 and UPV: 0.010455989544010455. We will include the results in the revised version of the paper. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comment 2: The writing can be further improved

Response:

We have inspected again the article to improve the clarity and coherence of our writing. Overall, we have focused on improving Section 3 (Method), including the explanation of our two main components: Section 3.1 (Semantic Retrieval Pipeline) and Section 3.2 (Silver Sentences Selection).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comments, Suggestions and Typos:

Comment 3: 

Missing References:

The following (earlier) works quantify, predict, and further analyzes the severity (changes) of mental illness over time with NLP techniques.

Li et al., 2018, Text-Based Detection and Understanding of Changes in Mental Health, SocInfo 2018.

Gaur et al., 2021, Characterization of time-variant and time-invariant assessment of suicidality on Reddit using C-SSRS, PLOS ONE 2021.

Response:

Thanks for the suggestion! We will look into these works and refer to similar studies considering different severity levels for mental health detection models.


% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! REVIEWER 3 !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 

First, we thank the reviewer for her/his feedback regarding our submission. We have done our best to address all the comments. We will comment point by point on our revisions. We are convinced that the revised manuscript is improved over the previous versions, particularly in the experimental analysis and further general explanations. The reviewer's appreciation has greatly contributed to this improvement. 

We appreciate its feedback on the paper, considering that our approach can be interpretable and explainable, and this fact can be helpful in clinical settings with appropriate validation of clinicians.


We will comment point by point on our revisions:

Comment 1: Sentence-level evaluation of the proposed method seems weak. Although Sec 5.1 and 5.2 discusses the quality of retrieved posts with only a handful of samples, a quantitative evaluation would be needed to assess how well different approaches in "silver sentence generation" retrieved similar posts. Manual annotations (such as the one carried out in the Aug Dataset approach) of sample silver sentences could be an option.

Response:

Thanks for the suggestion. To get statistics on a quantitative evaluation of our sentence selection models, we will use the manual annotations, as you point out. In specific, a total of 17.15\% were annotated as positives from the pool of candidate sentences. We will incorporate these results in the revised version of the paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comment 2: It is less discussed why the proposed method did not perform great with the larger dataset (eRisk 2021). Table 4 shows that the proposed methods outperformed the prior methods in the DCHR metric only. Furthermore, the proposed methods performed almost similarly between eRisk 2020 and 2021 even though the eRisk 2021's training set is nearly five times larger than that of 2020. Intuitively speaking, a retrieval-based method could work better if the source dataset was larger, because there would be more relevant examples. Does this mean the proposed method would not improve performance by increasing the size of training data?

Response:

We agree that intuitively, a retrieval system should improve its performance as training data increases. However, in a domain as complex as the detection of depression severity levels, it can be very difficult to obtain more general results. This has also been the case for the other participants in the eRisk collection, as most of the models have worsened results for the eRisk 2021 collection (for more details, please refer to the eRisk 2020 and 2021 working notes [1,2]).

In turn, this problem of generalization to different collections for these types of mental health detection models has been demonstrated in a recent study [3]. For this reason, we believe that not worsening the results, if not maintaining them, is not as strange a statistic as it might be in collections of a more standard nature.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Comments, Suggestions And Typos:

Comment 3: a) The terminology needs to be more accurate.

            The severity scale of the symptom is referred to as different words, 'option' and 'label', without notice. One coherent term is preferred for readability.
            "Silver sentence generation" (Sec 3.2 ) does not generate texts from scratch (like by using text generation models) but labels a pool of existing sentences afterwards. Consider using "distant supervision" or similar terms instead of "generation'.


Response: 
            We have changed our terminology to make the article easier to read. Regarding the term referred to the severity scale of a symptom, we now use the term "label" consistently. Moreover, we clarify this terminology in Footnote 3 (Page 3 of the manuscript).

            We have also changed the title of our sentence selection method (Subsection 3.2, now renamed to Silver Sentences Selection). Thank you for this appreciation! We agree that this term can generate confusion with text generation models. Therefore, we have changed the name of our sentence selection method.
            

Comment 4: b) What semantic similarity method was adopted in the "Aug Dataset" approach for "silver sentence generation"? Is it the same RoBERTa used in the "semantic retrieval pipeline"?


Response:

            Yes, we have used the same similarity method to augment silver sentences, which was a missing detail in the original manuscript. The revised version now includes an explicit mention of this important information.


Comment 5: c) The gold sentences (35 labelled sentences per symptom) could be made public to contribute to the community.

Response:

          Yes, we agree that this type of dataset may help develop depression detection models. We are currently working on a manuscript where we extend and analyze this resource in more detail. Following eRisk policies (the eRisk collections are the original data source), and due to the sensitivity of the data, the extended dataset will be available under a research data agreement.


Comment 6: d) In Table 4, the best RMSE in eRisk 2021 is 12.78 of CYUT, although 14.17 by a proposed method (Accum Voting SBERT) is marked in bold.

Response:

        We apologize for the error. The revised paper now correctly displays the best RMSE, highlighted in bold, for CYUT.

Comment 7: e) The discussion in Sec 5 should include ADODL and ACR. (On the other hand, the oracle experiment for AHR was very informative.)


Response:

            The ADODL is the Difference Between Overall Depression Levels (DODL) averaged over all users. DODL, does not look at question-level hits or differences but computes the overall depression level (sum of all the answers) for the real and automated questionnaires, and, next, the absolute difference (ad overall) between the real and the automated score is computed. Depression levels are integers between 0 and 63; thus, DODL is normalised into [0,1] as follows: DODL = (63 − ad overall)/63. For this metric, in eRisk2020, our proposed methods outperform all prior work. Similar to other metrics, our results are more modest in the eRisk2021 collection. This metric is quite similar to the RMSE, which considers the total error between the real and automated questionnaires. We considered not discussing this metric for page limit constraints in the Section.

            The ACR is the Closeness Rate (CR) averaged over all users. CR takes into account that the answers to the depression questionnaire represent an ordinal scale. Imagine that the actual user answered ”0”. A system S1, whose answer is ”3”, should be penalised more than a system S2, whose answer is ”1”. For each question, CR computes the absolute difference (ad) between the real and the automated answer (e.g. ad=3 and ad=1 for S1 and S2, respectively) and, next, this absolute difference is transformed into an effectiveness score as follows: CR = (mad − ad)/mad, where mad is the maximum absolute difference, which is equal to the number of possible answers minus one. As we argued in Section 5 (Results), we decided to focus more on assessing overall depression levels (DCHR metric), than focusing on specific symptoms.

            

            

            


Comment 8:

        f) The term "significantly" (at Line 554) should not be used in results/discussion sections unless it means statistically significant with a statistical test.

Response:

        We agree that this term can be confusing. We will remove it in the updated version of the article. Thanks again for going into so much detail.

Comment 9:

        g) Table 7's "Golden option" and "Predicted option" columns look the other way around according to the corresponding body text (Sec 5.2; the description at Line 560-561 does not match the table's values).

Response:

        That is correct. We apologize for the mistake. In the updated version, you will find the corrected column names.

[1] Losada, David E., Fabio Crestani, and Javier Parapar. "Overview of eRisk at CLEF 2020: Early Risk Prediction on the Internet (Extended Overview)." CLEF (Working Notes) (2020).

[2] Parapar, J., Martín-Rodilla, P., Losada, D. E., & Crestani, F. (2021). Overview of eRisk at CLEF 2021: Early Risk Prediction on the Internet (Extended Overview). CLEF (Working Notes), 864-887.

[3] Harrigian, Keith, Carlos Aguirre, and Mark Dredze. "Do models of mental health based on social media data generalize?." Findings of the association for computational linguistics: EMNLP 2020. 2020.

        




           
            



            
        

    


 




































